PLOT: Text-based Person Search with Part Slot Attention for Corresponding Part Discovery

Text-based person search, employing free-form text queries to identify individuals within a vast image collection, presents a unique challenge in aligning visual and textual representations, particularly at the human part level. Existing methods often struggle with part feature extraction and alignment due to the lack of direct part-level supervision and reliance on heuristic features. We propose a novel framework that leverages a part discovery module based on slot attention to autonomously identify and align distinctive parts across modalities, enhancing interpretability and retrieval accuracy without explicit part-level correspondence supervision. Additionally, text-based dynamic part attention adjusts the importance of each part, further improving retrieval outcomes. Our method is evaluated on three public benchmarks, significantly outperforming existing methods.

==> _macros.tex <==
% ---------------------------------------------------------------
% Other packages

% Commonly used abbreviations (\eg, \ie, \etc, \cf, \etal, etc.)
\usepackage{eccvabbrv}

% Include other packages here, before hyperref.
\usepackage{graphicx}
\usepackage{amsmath}	
\usepackage{amssymb}	
\usepackage{booktabs}
\usepackage{times}
\usepackage{microtype}
\usepackage{epsfig}
\usepackage{caption}
\usepackage{float}
\usepackage{placeins}
\usepackage{color, colortbl}
\usepackage{stfloats}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{xstring}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{url}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage[hang,flushmargin]{footmisc}
\usepackage{pifont}
\usepackage{wrapfig}
% \usepackage[novbox]{pdfsync}
% \usepackage[table,xcdraw,dvipsnames]{xcolor}

% for table
\usepackage{siunitx,booktabs}
\usepackage{newtxtext,newtxmath}

% The "axessiblity" package can be found at: https://ctan.org/pkg/axessibility?lang=en
\usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.
% \usepackage[review,year=2024,ID=03209]{eccv}

\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\hh}{- \ \ \ / \ \ \ -}
\newcommand{\quhqu}{ \ \ - \ \ }


\def\ie{\emph{i.e.}}
\def\eg{\emph{e.g.}}
\def\etal{\emph{et al.}}
\def\wrt{\emph{w.r.t.}}

\definecolor{black}{rgb}{0, 0, 0}
\definecolor{grn}{rgb}{0.1, 0.6, 0.1}
\definecolor{mgt}{rgb}{0.6, 0.1, 0.6}
\definecolor{red}{rgb}{0.7 0.1 0.1}
\definecolor{blue}{rgb}{0.0 0.0 1.0}
\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{Gray}{gray}{0.9}
\definecolor{grey}{rgb}{0.9, 0.9, 0.9}
\newcommand{\ccol}{\cellcolor{grey}}
% \usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\expnum}[2]{{#1}\mathrm{e}{-#2}}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand{\sftype}[1]{{\textsf{\small #1}}}

%\newcommand{\jicheol}[1]{{\color{blue}{#1}}}
\newcommand{\jicheol}[1]{{\color{black}{#1}}}
\newcommand{\boseung}[1]{{\color{black}{#1}}}
\newcommand{\bs}[1]{{\color{black}{#1}}}
\newcommand{\suha}[1]{{\color{black}{#1}}}
\newcommand{\suhac}[1]{{\color{black}{(#1)}}}
%\newcommand{\dw}[1]{{\color{grn}{#1}}}
\newcommand{\dw}[1]{{\color{black}{#1}}}

==> eccv_header.tex <==
% ---------------------------------------------------------------
% Include basic ECCV package
% TODO REVIEW: Insert your submission number below by replacing '*****'
% TODO FINAL: Comment out the following line for the camera-ready version
\usepackage[review,year=2024,ID=03209]{eccv}
% TODO FINAL: Un-comment the following line for the camera-ready version
\usepackage{eccv}
 
% OPTIONAL: Un-comment the following line for a version which is easier to read
% on small portrait-orientation screens (e.g., mobile phones, or beside other windows)
%\usepackage[mobile]{eccv}
 \input{_macros}

% ---------------------------------------------------------------

% Hyperref package

% It is strongly recommended to use hyperref, especially for the review version.
% Please disable hyperref *only* if you encounter grave issues.
% hyperref with option pagebackref eases the reviewers' job, but should be disabled for the final version.
%
% If you comment hyperref and then uncomment it, you should delete
% main.aux before re-running LaTeX.
% (Or just hit 'q' on the first LaTeX run, let it finish, and you
%  should be clear).

% TODO FINAL: Comment out the following line for the camera-ready version
% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}
\usepackage[pagebackref,breaklinks,colorlinks,citecolor=eccvblue]{hyperref}

% TODO FINAL: Un-comment the following line for the camera-ready version
%\usepackage{hyperref}

% Support for ORCID icon
\usepackage{orcidlink}




==> figures/fig_encoder_decoder.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/CVPR24_encoder_decoder.pdf}
    \vspace{-1mm}   
    \caption{Details of encoder-decoder architecture.}
    \label{fig:encoder_decoder}
    \vspace{-5mm}
\end{figure}

==> figures/fig_loss.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/CVPR24_loss.pdf}
    % \vspace{1mm}   
    \caption{A conceptual illustration of the Comanality-based Margin Ranking (CMR) loss function in Eq.~\eqref{eq:cmr loss}. The square and circle symbols denote the fine embeddings of image and text modalities, respectively.}
    \label{fig:Loss}
    \vspace{-3mm}
\end{figure}

==> sections/01_intro_backup.tex <==
\section{Introduction}
\label{sec:intro}

\iffalse
Person search is the task of finding individuals within a vast collection of images based on queries describing visual characteristics of target in images~\cite{Sun_2018_ECCV, Kalayeh_2018_CVPR, Ali_2018_ECCV, Zhong_2018_CVPR, Wang_2018_ECCV}, attribute sets~\cite{yin2017adversarial, dong2019person, cao2020symbiotic, jeong2021asmr}, and natural language~\cite{li2017person, li2017identity, zhang2018deep, gao2021contextual, ding2021semantically, suo2022simple}.
It has played vital roles in public safety applications, such as identifying criminals in videos and finding missing people using multiple surveillance cameras that have non-overlapping fields of view.

Text-based person search refers to the person search task that employs free-form text as query. %to retrieve individuals within a large collection of images.
This task enables efficient and effective person search thanks to the flexible and user-friendly query acquisition.
Also, text queries are often more suitable for person search in the wild than other types of queries such as images~\cite{Sun_2018_ECCV, Kalayeh_2018_CVPR} and attributes~\cite{yin2017adversarial, jeong2021asmr}; Image queries are not accessible when eyewitness memory is the only evidence for identification, and the expression power of attribute-based queries is restricted strictly by a predefined set of attributes.
\fi

% Person search is the task of identifying individuals in a large image set given queries that describe visual characteristics of target through image~\cite{Sun_2018_ECCV, Kalayeh_2018_CVPR}, attributes~\cite{yin2017adversarial, jeong2021asmr}, and free-form text~\cite{li2017person, li2017identity, zhang2018deep, gao2021contextual, ding2021semantically, suo2022simple, irra}.
% Text-based person search refers to the person search task that employs free-form text as query.
% Text queries are more feasible in terms of query acquisition than image queries, and provide more expressive versatility than attribute queries, making them more suited for real-world applications.

\jicheol{
Text-based person search is the task of identifying the target person from the vast collection of images with a free-form text query.
This task requires extracting identifiable features, such as human parts, from both textual and visual modalities.
Then, the alignment of correspondence between the extracted human part features across modalities is essential for text-based person search.
%Then, it is essential to ensure that the extracted human part features align correspondingly across modalities for retrieval.
However, without part-level supervision, the extraction and alignment of these part features from free-form text and images become significantly challenging.


\input{figures/fig_arch}


To address this challenge, previous work~\cite{chen2022tipcb, suo2022simple} relies on the heuristic part features obtained by equi-horizontally cropping the entire image because there are no straightforward methods to extract part features in free-form text queries. 
Then they transform and assign the free-form text queries to each heuristic visual part feature through several networks.
However, this approach is constrained by the limitations of heuristic part visual features that are susceptible to deformation caused by occlusion and pose variation.
To move beyond the heuristic visual parts, some earlier work~\cite{jing2020pose, wang2020vitaa, lgur} proposed a learning-based approach for part feature extraction.
Nevertheless, these methods tend to generate redundant part features that lack disentanglement~\cite{lgur}, or they require access to additional part-level supervisions~\cite{jing2020pose, wang2020vitaa}.
}

\iffalse
\dw{
%[Needs of part feature for person ReID]
% target person 찾기 위한 세밀한 비교가 어렵다, part-level supervision이 존재하지 않기 때문에 세밀한 비교를 위한 part feature 추출이 어려워서 
% 같은 semantic category인 person안에서의 fine-grained difference? subtle differrence를 포착해야 하기 때문에?
% Query description; 찾고자 하는 사람에 대한 설명은, 보통 특징적인 part 서술의 집합으로 이루어진다.
Most of previous work~\cite{chen2022tipcb, suo2022simple, jing2020pose, wang2020vitaa, lgur, ivt } in person search employ part-level representation of data as a crucial initial stage. 
This approach is motivated by the necessity to recognize subtle differences between individuals, which are often discernible at the part-level (\eg blah blah blah). 
% It is because the person search requires the awareness of subtle difference between individuals, and the differences between person usually can be spotted within part level (\eg blah blah blah).
This need is particularly evident in text-based person search, where queries may not provide a comprehensive description of individuals but instead focus on distinctive parts. 
Therefore, employing part features empowers a model to effectively find the target individual, even when dealing with fine-grained differences and partial descriptions.

[Why obtaining visual part feature is challenging]
% visual part를 어떻게 찾을 수 있는가?
% 기존에도 part based approach가 있었으나, 좀 naive하다는 것을 말해주면 될 것 같음.
However, to obtain part features from images, previous work often relies on the heuristic involving equi-horizontally cropping of the entire image~\cite{chen2022tipcb, suo2022simple}.
These methods are susceptible to deformation caused by occlusion and pose variation.
In contrast, some earlier work~\cite{jing2020pose, wang2020vitaa, lgur} proposed a learning-based approach for part feature extraction.
Nevertheless, these methods tend to generate redundant part features that lack disentanglement~\cite{lgur}, or they require access to an external part segmentation dataset~\cite{jing2020pose, wang2020vitaa}.

% Although using free-form text as query for person search offers distinct advantages over attribute or image query, they pose additional challenges in extracting part features. 
% textual part를 어떻게 찾을 수 있는가?
% 기존에도 attribute based approach가 있었으나, 좀 naive하다는 것을 말해주면 될 것 같음.
% Previous research in person search using images or pre-defined attribute sets as queries has typically focused on extracting part features to discern subtle differences across people. 
[Why obtaining textual part feature is challenging]
While utilizing free-form text queries offers distinct advantages, the extraction of part features from such text queries presents two additional challenges. 
Firstly, there are no straightforward methods to extract part features from free-form text queries, as descriptions of the same part can be conveyed in countless ways, and the order of these descriptions within a sentence is arbitrary.
%(Needs further supplement about which heuristics are used in previous literature)
Moreover, unlike attribute queries where each attribute is associated with one of the predefined part categories, it remains unknown which human part each word or phrase in the text query describes.
Thereby, the model should not only discover part features from the free-form text but also infer the latent correspondences between the textual and visual part features.
\jicheol{%In previous work~\cite{ivt}, part features are selectively extracted based on the parts of speech of words in the text description.
%Moreover, it remains unknown which human part is described by each word or phrase in the text description, due to the heuristic part extraction approach.
%Thereby, we should not only discover part features from the free-form text but also infer the latent correspondences between the textual and visual part features.
}
% Thereby, the model needs to not only discover part description from the free-form text, but also infer the latent part correspondence with the visual part features.
% which makes impossible employing simple heuristics as done for image~\cite{}.
% Applying heuristics as done for images is not available since the order of part description in text query is arbitrary. 
% In the case of attribute sets, predefined part-level attribute labels are directly employed to encode part-specific features, aiding in capturing the subtle differences among individuals.
% However, when it comes to text-based person search with free-form text as queries, unlike attribute sets, there is no part-level supervision available. 
% Also, obtaining na\"ive segmented part features from text queries is not as straightforward as it is in the image modality.
}
\fi

\jicheol{
To tackle the above issues, we introduce a new framework that can discover distinctive part features in both modalities and align them without any correspondence supervision; its overall architecture is illustrated in Fig.~\ref{fig:architecture}.
% \iffalse
% \dw{In order to extract distinctive part features from both modalities, we employ a slot attention~\cite{slot} module for each modality, following their respective backbone models.
% Specifically, within the slot attention mechanism, a set of embedding vectors, termed \emph{part slots}, undergo refinement to form the part features that represent distinct parts in the input data. %present in the input data.
% %, which can contain information related to distinct human parts that are shared between two modalities
% These part slots engage in an iterative attention process, competing amongst themselves to bind with the input features.
% To ensure correspondence between part slots from different modalities, we share the part slots within the visual and textual modalities.
% During training and evaluation, part embeddings from the same part slots are regarded to represent the identical part semantics.
% Consequently, the proposed framework can decompose raw images or text queries into a set of part embeddings, establishing correspondence between them without the need for explicit part labels.}
% \fi
% \iffalse
% \jicheol{To extract distinctive part features from both modalities, we employ a slot attention~\cite{slot} module for each modality, following their respective backbone models.
% Specifically, within the slot attention mechanism, a set of embedding vectors, termed \emph{part slots}, can contain primitive information related to human parts that are shared between two modalities.
% These part slots undergo refinement through several iterative attention processes, where they compete amongst themselves to bind with the input data, ultimately refining the part slots as part features, termed \emph{part embeddings}, represent distinct parts in the input data.
% To ensure correspondence between part embeddings from different modalities, we share the part slots within the visual and textual modalities.
% During training and evaluation, part embeddings from the same part slots represent the semantics of identical part.
% Consequently, the proposed framework can decompose raw images or text queries into a set of part embeddings, where the correspondence between them is established without the explicit part labels. 
% }
% \fi
To extract distinctive part features from both modalities, we introduce a part discovery module based on the slot attention mechanism~\cite {slot} for each modality, following their respective backbone models.
Slot attention is an attention mechanism designed for object-centric learning, which segments input data into a set of slots representing individual entities without requiring object-level supervision. 
%This process allows slots to iteratively compete for aggregating input data, ensuring unique representations for each entity.
In the proposed part discovery module, we first define a set of learnable embedding vectors, termed \emph{part slots}, that contain primitive information related to human parts shared between two modalities.
Then, these part slots undergo refinement through several iterative attention processes, where they compete amongst themselves to bind with the input data; ultimately, the part slots are transformed into part features, termed \emph{part embeddings}, that represent distinctive parts in the input data.

% [interpretability]
To ensure correspondence between part embeddings from different modalities, we share the part slots within the visual and textual modalities.
% The part slots are shared within the visual and textual modalities, ensuring correspondence between part embeddings from different modalities.
During training and evaluation, part embeddings from the same part slots represent the semantics of the identical part.
Consequently, thanks to the correspondence of part embeddings extracted by shared part slots, it enables an interpretable retrieval system.
%Consequently, the proposed part discovery module can decompose raw images or text queries into a set of part embeddings, where the correspondence between them is established without the explicit part labels.
}
\iffalse
\dw{
To tackle the challenges for obtaining part features, we propose the part discovery module, which can obtain the representation for each part without relying on the heuristics or additional supervision.
In part discovery module, learnable embedding vectors termed \emph{part slots} iteratively compete with each other for aggregating the input data.
Parts slots are shared between visual and textual modalities, 
}
\fi
% \iffalse
% \jicheol{To tackle the above issues, we introduce a framework that can discover part related representation in both modalities and align those without any correspondence supervision.
% To be specific, although features of the two modalities are computed by separate backbone models, they are aggregated into a fixed number of feature vectors by employing slot attention~\cite{}—a recursive attention mechanism that yields a set of feature vectors termed \emph{slots}.
% These slots engage in an iterative competition, vying for binding to distinct parts of the input features.
% In order to extract distinctive part features from both modalities, we have a slot attention module for each modality, following their respective backbone models. 
% To capture the same entity from inputs of the two different modalities and establish correspondence between them, we initialize the slots with shared learnable parameters across modalities and match the same slots from different modalities.}
% \fi

\jicheol{
% [Text-based Dynamic Part Attention]
Furthermore, we introduce a new similarity aggregation method for part embeddings called text-based dynamic part attention (TDPA) pooling, which dynamically adjusts the weights of part embeddings based on the text query.
Given a text query as input, TDPA predicts the importance weight of each slot for retrieval and applies the predicted importance weights to aggregate the similarities of part embeddings between two modalities.
It allows for the adaptive assignment of importance to each part embedding based on each text query.
\iffalse
However, since the proposed part discovery module decomposes the input data exhaustively, some part embeddings may convey less significant information (e.g., stop words or punctuation in text).
To address above issue, we propose a new similarity aggregation method called text-based dynamic part attention (TDPA) pooling, which dynamically adjusts the weights of part embeddings based on the text query.
Given a text query as input, TDPA predicts the importance weight of each slot for retrieval, and applies the predicted importance weights to aggregate the similarities of part embeddings between two modalities.
%It reduces the influence of no-informative part features (e.g., background in images or punctuation in text) and allows for the adaptive assignment of importance to each part feature based on each text query.
It reduces the influence of non-informative part embeddings (e.g., stop words or punctuation in text) and allows for the adaptive assignment of importance to each part slot based on each text query.
%Hence, diminishes the impact of less significant part features and promotes a more informative retrieval that reflects important semantic similarity.
\fi
}

\iffalse
\jicheol{[Interpretability with part-level cross-modal correspondence]
%Additionally, the established correspondence of the part slots provides intuitive interpretability.
%For instance, by utilizing the attention of part slots for a given text query, it identifies which part slot is interested in a specific set of text, and by examining the corresponding part slot attention in the opposite modality, one can view the areas of interest in the image.
%Consequently, in the inference, the framework allows users to modify the interest of specific slots, enabling a user-customized text-based person search.
Additionally, the established correspondence of part embeddings between modalities provides intuitive interpretability.
For instance, by utilizing the attention of part embeddings for a given text query, it identifies which part slot is interested in a specific human part.
Furthermore, it allows users to modify the interest of specific slots, enabling a user-customized text-based person search in which specific human part can be prioritized for retrieval.
The proposed framework introduces a method termed text-based dynamic part attention (TDPA), which dynamically adjusts the weights of part embeddings based on the text query, thereby enhancing the performance of text-based person search.
Given a text query as input, our framework predicts the importance weight of each slot for retrieval, and applies the predicted importance weights to aggregate the similarities of part embeddings between two modalities.
%It reduces the influence of no-informative part features (e.g., background in images or punctuation in text) and allows for the adaptive assignment of importance to each part feature based on each text query.
It reduces the influence of no-informative part embeddings (e.g., stop words or punctuation in text) and allows for the adaptive assignment of importance to each part slot based on each text query.
Hence, diminishes the impact of less significant part features and promotes a more informative retrieval that reflects important semantic similarity.
}
\fi

\iffalse
\dw{[Explanation for global feature and part feature?]}

% In our method, we calculate the similarity between corresponding slots across different modalities and aggregate these similarities into a single one. 
\dw{The similarity between image and text query is measured by aggregating the similarity between the global feature and each part feature. 
Yet, since the employed slot attention mechanism decomposes the input data exhaustively, some part features may convey less significant information (e.g., background in images or punctuation in text).
Involving such no-informative part features for similarity measurement will degrade the accuracy of the person search.
To address this challenge, we introduce learnable weights to aggregate the part-wise similarities.
These learnable weights enable us to adaptively assign importance to each part feature, which reduces the impact of less significant part features and promotes a more informative similarity measurement that reflects accurate semantic similarity.}
\fi

\iffalse
\jicheol{In our method, we calculate the similarity between corresponding slots across different modalities and aggregate these similarities into a single one. 
Yet, the part-competitive nature of slot attention introduces a challenge where some slots may convey less significant information (e.g., background in images or punctuation in text), hindering the performance of person search.
To address this challenge, we introduce learnable weights for the aggregation of slot-specific similarities.
These learnable weights enable us to adaptively assign importance to each slot, reducing the impact of less significant slots and promoting a more meaningful aggregation through a weighted sum.}
\fi

% With our proposed method, we can extract part features that correspond between modalities without part-level supervision in both image and text modalities.
% Additionally, our method tackles concerns stemming from a straightforward part feature extraction in image modality; the even division of image regions does not guarantee comprehensive coverage of body parts and introduces noise due to the including background.

Our method was evaluated and compared with prior work on three public benchmarks~\cite{li2017person, ding2021semantically, zhu2021dssl}, where it clearly outperformed all existing methods thanks to the rich representation based on part embeddings.
The main contribution of our work is three-fold:
\begin{itemize}
   \vspace{-1mm}\item We introduce a new architecture for text-based person search that discovers human part features termed part embeddings aligned between the two modalities without part-level supervision.
   \item Thanks to the characteristics of the proposed part embeddings, it is possible to conduct an interpretable text-based person search.
   \item Additionally, we introduce a novel similarity aggregation method for part embeddings that adaptive assignment of importance to each part embedding based on each text query.
\end{itemize}

% However, the advantages of text queries come with an additional challenge, the large gap between image and text modalities. 
% Due to this modality gap, it becomes even more difficult to establish correspondences between target and query, 
% and consequently to distinguish subtle differences across people.

% To overcome the modality gap, prior studies have employed joint image-text embedding that aims at representing data of both modalities in a common embedding space~\cite{frome2013devise, kiros2014unifying, faghri2017vse++}.
% They have emphasized in particular the development of loss functions to mitigate the modality gap.
% However, they have not paid sufficient attention to the model architecture design for reducing the gap during the encoding process of each modality, and thus leave room for further improvement.


==> tables/tab_ablation_aggregation.tex <==
% \begin{wraptable}{r}{5.5cm}
%     \caption{Comparison to TIPCB (a) and Performance of our method with different similarity aggregation strategies (b) on the CUHK-PEDES dataset.}
%     % \vspace{-2mm}
%     \label{tab:ablation_similarity_aggregation}
%     \resizebox{0.46\textwidth}{!}{%   
%     \begin{tabular}{c|lccc}
%     \toprule
%     \multicolumn{1}{c}{}&\multicolumn{1}{l}{\textbf{Methods}}  & R@1 & R@5 & R@10\\ [-0.3ex]  \midrule
%     \multirow{1}{*}{(a)} & Ours + TIPCB~\cite{chen2022tipcb} & 73.23 &  89.10 & 94.04 \\ \midrule
%     \multirow{2}{*}{(b)} &Cumulative Aggregation & 73.96& 89.73 & 93.84\\
%     &Static Aggregation & 74.33 & 89.44 & 93.52 \\ \midrule
%     \multicolumn{1}{c}{}&\multicolumn{1}{l}{Ours}& \textbf{75.28} & \textbf{90.42} & \textbf{94.12} \\ \bottomrule
%     \end{tabular}
%     }
% \end{wraptable}

\begin{table}[t!]
    \centering
    \caption{Comparison to TIPCB (a) and Performance of our method with different similarity aggregation strategies (b) on the CUHK-PEDES dataset.}
    \vspace{-2mm}
    % \resizebox{0.46\textwidth}{!}{%   
    \begin{tabular}{c|lccc}
    \toprule
    \multicolumn{1}{c}{}&\multicolumn{1}{l}{\textbf{Methods}}  & R@1 & R@5 & R@10\\ [-0.3ex]  \midrule
    \multirow{1}{*}{(a)} & Ours + TIPCB~\cite{chen2022tipcb} & 73.23 &  89.10 & 94.04 \\ \midrule
    \multirow{2}{*}{(b)} &Cumulative Aggregation & 73.96& 89.73 & 93.84\\
    &Static Aggregation & 74.33 & 89.44 & 93.52 \\ \midrule
    \multicolumn{1}{c}{}&\multicolumn{1}{l}{Ours}& \textbf{75.28} & \textbf{90.42} & \textbf{94.12} \\ \bottomrule
    \end{tabular}
    % }
    \label{tab:ablation_similarity_aggregation}
\end{table}

==> tables/tab_comp_irra_tipcb.tex <==
\begin{table}[!ht]
    \centering
    \caption{Performance of our method with different pooling methods and a variant of ours with applying CMR loss at coarse embeddings on the CUHK-PEDES dataset.}
    \vspace{-2mm}
    \resizebox{0.46\textwidth}{!}{%   
    \begin{tabular}{c|l|c|c|c}
    \toprule
    \multicolumn{2}{l|}{Method}  & R@1 & R@5 & R@10\\ \midrule
    \multirow{1}{*}{(a)} & Coarse with CMR & 64.99&  83.40 & 88.82 \\ \midrule
    \multirow{2}{*}{(b)} &GAP & 62.20& 81.45 & 87.65\\
    % &GMP (ours) & 65.64 & 83.40 & 89.42 \\ 
    &GAP+GMP & 65.12 & 82.70 & 88.81 \\ \midrule
    \multicolumn{2}{c|}{Ours}& \textbf{65.64} & \textbf{83.40} & \textbf{89.42} \\ \bottomrule
    \end{tabular}
    }
    \label{tab:comp_irra_tipcb}
\end{table}
